When Do Graph Neural Networks Help with Node Classification? Investigating the Impact of Homophily Principle on Node Distinguishability

Homophily principle, i.e., nodes with the same labels are more likely to be connected, has been believed to be the main reason for the performance superiority of Graph Neural Networks (GNNs) over Neural Networks on node classification tasks. Recent research suggests that, even in the absence of homophily, the advantage of GNNs still exists as long as nodes from the same class share similar neighborhood patterns. However, this argument only considers intra-class Node Distinguishability (ND) but neglects inter-class ND, which provides incomplete understanding of homophily on GNNs. In this paper, we first demonstrate such deficiency with examples and argue that an ideal situation for ND is to have smaller intra-class ND than inter-class ND. To formulate this idea and study ND deeply, we propose Contextual Stochastic Block Model for Homophily (CSBM-H) and define two metrics, Probabilistic Bayes Error (PBE) and negative generalized Jeffreys divergence, to quantify ND. With the metrics, we visualize and analyze how graph filters, node degree distributions and class variances influence ND, and investigate the combined effect of intra- and inter-class ND. Besides, we discovered the mid-homophily pitfall, which occurs widely in graph datasets. Furthermore, we verified that, in real-work tasks, the superiority of GNNs is indeed closely related to both intra- and inter-class ND regardless of homophily levels. Grounded in this observation, we propose a new hypothesis-testing based performance metric beyond homophily, which is non-linear, feature-based and can provide statistical threshold value for GNNs' the superiority. Experiments indicate that it is significantly more effective than the existing homophily metrics on revealing the advantage and disadvantage of graph-aware modes on both synthetic and benchmark real-world datasets.

==> Rebuttal/Author_Rebuttal <==
In this part, we will provide experimental results of Label Informativeness (LI) and adjusted homophily ($H_\text{adj}$) on small- and large-scale datasets and compare them with the proposed metrics. Before discussing the results, we would like to introduce 2 threshold values for classifier-based performance metrics (you can find it in Appendix G.2)

Typically, the threshold for homophily and heterophily graphs is set at 0.5. For classifier-based performance metrics, we establish two benchmark thresholds as below,
 • Normal Threshold 0.5 (NT0.5): Although not indicating statistical significance, we are still comfortable to set 0.5 as a loose threshold. A value exceeding 0.5 suggests that the G-aware model is not very likely to underperform their coupled G-agnostic model on the tested graph and vice versa. (Error cases with regard to NT0.5 are marked by grey)
 • Statistical Significant Threshold 0.05 (SST0.05): Instead of offering an ambiguous statistical interpretation, SST0.05 will provide a clear statistical meaning. A value smaller than 0.05 implies that the G-aware model significantly underperforms their coupled G-agnostic model and a value greater than 0.95 suggests a high likelihood of G-aware model outperforming their coupled G-agnostic model. Besides, a value ranging from 0.05 to 0.95 indicates no significant performance distinction between G-aware model and its G-agnostic model. SST0.05 is a more strict threshold than NT0.5. Therefore, we will observe more error cases under SST0.05 than NT0.5. (Error cases with regard to SST0.05 are marked by red)

We can see that, no matter on small- or large-scale datasets, the classifier-based performance metrics (CPMs) are significantly better than the existing metrics on revealing the advantages and disadvantages of GNNs, decreasing the overall error rate from at least 0.34 to 0.13 (at most 0.19 under SST0.05).

==> rebuttal_tab_inter_inner_euclidean_distance_hypothesis_testing.tex <==
% Table generated by Excel2LaTeX from sheet 'Distance Ratio'
\begin{table*}[htbp]
  \centering
  \caption{P-values, homophily values and classifier-based performance metrics on 9 real-world benchmark datasets. Cells marked by grey are incorrect results for both SGC v.s. MLP-1 and GCN v.s. MLP-2 and cells marked by blue are incorrect for 1 of the 2 tests. We use 0.5 as the threshold value of the homophily metrics.}
  \resizebox{1\hsize}{!}{
   \begin{tabular}{c|c|ccccccccc}
    \toprule
    \toprule
          &       & Cornell & Wisconsin & Texas & Film  & Chameleon & Squirrel & Cora  & CiteSeer & PubMed \\
    \midrule
          & $\text{H}_\text{edge}$ & \cellcolor[rgb]{ .647,  .647,  .647}0.5669 & 0.4480 & 0.4106 & 0.3750 & \cellcolor[rgb]{ .647,  .647,  .647}0.2795 & \cellcolor[rgb]{ .647,  .647,  .647}0.2416 & 0.8100 & 0.7362 & \cellcolor[rgb]{ .357,  .608,  .835}0.8024 \\
     & $\text{H}_\text{node}$ & 0.3855 & 0.1498 & 0.0968 & 0.2210 & \cellcolor[rgb]{ .647,  .647,  .647}0.2470 & \cellcolor[rgb]{ .647,  .647,  .647}0.2156 & 0.8252 & 0.7175 & \cellcolor[rgb]{ .357,  .608,  .835}0.7924 \\
    {Baseline} & $\text{H}_\text{class}$ & 0.0468 & 0.0941 & 0.0013 & 0.0110 & \cellcolor[rgb]{ .647,  .647,  .647}0.0620 & \cellcolor[rgb]{ .647,  .647,  .647}0.0254 & 0.7657 & 0.6270 & \cellcolor[rgb]{ .357,  .608,  .835}0.6641 \\
    { Homophily} & $\text{H}_\text{agg}$ & \cellcolor[rgb]{ .647,  .647,  .647}0.8032 & \cellcolor[rgb]{ .647,  .647,  .647}0.7768 & \cellcolor[rgb]{ .647,  .647,  .647}0.694 & \cellcolor[rgb]{ .647,  .647,  .647}0.6822 & 0.61  & \cellcolor[rgb]{ .647,  .647,  .647}0.3566 & 0.9904 & 0.9826 & \cellcolor[rgb]{ .357,  .608,  .835}0.9432 \\
          { Metrics}& $\text{H}_\text{GE}$ & 0.31  & 0.34  & 0.35  & 0.16  & \cellcolor[rgb]{ .647,  .647,  .647}0.0152 & \cellcolor[rgb]{ .647,  .647,  .647}0.0157 & \cellcolor[rgb]{ .647,  .647,  .647}0.17 & \cellcolor[rgb]{ .647,  .647,  .647}0.19 & \cellcolor[rgb]{ .357,  .608,  .835}0.27 \\
    & $\text{H}_\text{adj}$ & 0.1889 & 0.0826 & 0.0258 & 0.1272 & \cellcolor[rgb]{ .647,  .647,  .647}0.0663 & \cellcolor[rgb]{ .647,  .647,  .647}0.0196 & 0.8178 & 0.7588 & \cellcolor[rgb]{ .357,  .608,  .835}0.7431 \\
    & $\text{LI}$    & 0.0169 & 0.1311 & 0.1923 & 0.0002 & \cellcolor[rgb]{ .647,  .647,  .647}0.048 & \cellcolor[rgb]{ .647,  .647,  .647}0.0015 & 0.5904 & \cellcolor[rgb]{ .647,  .647,  .647}0.4508 & \cellcolor[rgb]{ .357,  .608,  .835}0.4093 \\
    \midrule
    {Classifier-based } & $\text{KR}_\text{NNGP}$ & 0.00  & 0.00  & 0.00  & 0.00  & 1.00  & 1.00  & 1.00  & 1.00  & \cellcolor[rgb]{ .357,  .608,  .835}1.00 \\
    {Performance Metrics} & GNB & 0.00  & 0.00  & 0.00  & 0.00  & 1.00  & 1.00  & 1.00  & 1.00  & \cellcolor[rgb]{ .357,  .608,  .835}1.00 \\
    \midrule
    \multicolumn{1}{c|}{\multirow{4}[2]{*}{SGC v.s. MLP-1}} & p-value & 0.00  & 0.00  & 0.00  & 0.00  & 1.00  & 1.00  & 1.00  & 1.00  & 0.00 \\
          & ACC SGC & 70.98 $\pm$ 8.39 & 70.38 $\pm$ 2.85 & 83.28 $\pm$ 5.43 & 25.26 $\pm$ 1.18 & 64.86 $\pm$ 1.81 & 47.62 $\pm$ 1.27 & 85.12 $\pm$ 1.64 & 79.66 $\pm$ 0.75 & 85.5 $\pm$ 0.76 \\
          & ACC MLP-1 & 93.77 $\pm$ 3.34 & 93.87 $\pm$ 3.33 & 93.77 $\pm$ 3.34 & 34.53 $\pm$ 1.48 & 45.01 $\pm$ 1.58 & 29.17 $\pm$ 1.46 & 74.3 $\pm$ 1.27 & 75.51 $\pm$ 1.35 & 86.23 $\pm$ 0.54 \\
          & \textbf{Diff Acc} & -22.79 & -23.49 & -10.49 & -9.27 & 19.85 & 18.45 & 10.82 & 4.15  & -0.73 \\
    \midrule
    \multicolumn{1}{c|}{\multirow{4}[2]{*}{GCN v.s. MLP-2}} &  p-value & 0.00  & 0.00  & 0.00  & 0.00  & 1.00  & 1.00  & 1.00  & 1.00  & \cellcolor[rgb]{ .647,  .647,  .647}0.00 \\
          & ACC GCN & 82.46 $\pm$ 3.11 & 75.5 $\pm$ 2.92 & 83.11 $\pm$ 3.2 & 35.51 $\pm$ 0.99 & 64.18 $\pm$ 2.62 & 44.76 $\pm$ 1.39 & 87.78 $\pm$ 0.96 & 81.39 $\pm$ 1.23 & 88.9 $\pm$ 0.32 \\
          & ACC MLP-2 & 91.30 $\pm$ 0.70 & 93.87 $\pm$ 3.33 & 92.26 $\pm$ 0.71 & 38.58 $\pm$ 0.25 & 46.72 $\pm$ 0.46 & 31.28 $\pm$ 0.27 & 76.44 $\pm$ 0.30 & 76.25 $\pm$ 0.28 & 86.43 $\pm$ 0.13 \\
          & \textbf{Diff Acc} & -8.84 & -18.37 & -9.15 & -3.07 & 17.46 & 13.48 & 11.34 & 5.14  & 2.47 \\
    \bottomrule
    \bottomrule
    \end{tabular}%
    }
  \label{rebuttal_tab:hypothesis_testing_kernel_homo_performance_comparison}%
\end{table*}%

==> rebuttal_tab_large_datasets_results.tex <==
% Table generated by Excel2LaTeX from sheet 'Classifier-based'
\begin{table}[htbp]
  \centering
  \caption{Comparison on large-scale datasets}
  \resizebox{0.9\hsize}{!}{
    \begin{tabular}{c|c|ccccccc}
    \toprule
    \toprule
          &       & Penn94 &  pokec &  arXiv-year &  snap-patents &  genius &  twitch-gamers & Deezer-Europe \\
    \midrule
          & $\text{H}_\text{edge}$ & 0.4700 & 0.4450 & \cellcolor[rgb]{ .647,  .647,  .647}0.2220 & 0.0730 & \cellcolor[rgb]{ .647,  .647,  .647}0.6180 & \cellcolor[rgb]{ .647,  .647,  .647}0.5450 & \cellcolor[rgb]{ .647,  .647,  .647}0.5250 \\
     & $\text{H}_\text{node}$ & 0.4828 & 0.4283 & \cellcolor[rgb]{ .647,  .647,  .647}0.2893 & 0.2206 & \cellcolor[rgb]{ .647,  .647,  .647}0.5087 & \cellcolor[rgb]{ .647,  .647,  .647}0.5564 & \cellcolor[rgb]{ .647,  .647,  .647}0.5299 \\
    {Baseline} & $\text{H}_\text{class}$ & 0.0460 & 0.0000 & \cellcolor[rgb]{ .647,  .647,  .647}0.2720 & 0.1000 & 0.0800 & 0.0900 & 0.0300 \\
    {Homophily} & $\text{H}_\text{agg}$ & 0.2712 & 0.0807 & 0.7066 & \cellcolor[rgb]{ .647,  .647,  .647}0.6170 & \cellcolor[rgb]{ .647,  .647,  .647}0.7823 & 0.4172 & \cellcolor[rgb]{ .647,  .647,  .647}0.5580 \\
    {  Metrics} & $\text{H}_\text{GE}$ & 0.3734 & \cellcolor[rgb]{ .647,  .647,  .647}0.9222 & 0.8388 & \cellcolor[rgb]{ .647,  .647,  .647}0.6064 & \cellcolor[rgb]{ .647,  .647,  .647}0.6655 & 0.2865 & 0.0378 \\
    & $\text{H}_\text{adj}$ & 0.0366 & -0.1132 & \cellcolor[rgb]{ .647,  .647,  .647}0.0729 & 0.0907 & 0.1432 & 0.1010 & 0.1586 \\
    & $\text{LI}$    & 0.0851 & 0.0172 & \cellcolor[rgb]{ .647,  .647,  .647}0.0407 & 0.0243 & 0.0025 & 0.0058 & 0.0007 \\
    \midrule
    {Classifier-based } & $\text{KR}_\text{L}$ & 0.00  & 0.03  & 0.98  & \textcolor[rgb]{ 1,  0,  0}{0.19} & 0.00  & \textcolor[rgb]{ 1,  0,  0}{0.25} & 0.00 \\
    {Performance Metrics} & GBN & 0.00  & 0.00  & 1.00  & \cellcolor[rgb]{ .647,  .647,  .647}\textcolor[rgb]{ 1,  0,  0}{1.00} & 0.00  & \cellcolor[rgb]{ .647,  .647,  .647}\textcolor[rgb]{ 1,  0,  0}{1.00} & 0.00 \\
    \midrule
          & ACC SGC & 67.06 $\pm$ 0.19 & 52.88 $\pm$ 0.64 & 35.58 $\pm$ 0.22  & 29.65 $\pm$ 0.04 & 82.31 $\pm$ 0.45 & 57.9 $\pm$ 0.18 & 61.63 $\pm$ 0.25 \\
    {SGC vs MLP1} & ACC MLP-1 & 73.72 $\pm$ 0.5 & 59.89 $\pm$ 0.11 & 34.11 $\pm$ 0.17 & 30.59 $\pm$ 0.02 & 86.48 $\pm$ 0.11 & 59.45 $\pm$ 0.16 & 63.14 $\pm$ 0.41 \\
          & \textbf{Diff Acc} & -6.66 & -7.01 & 1.47  & -0.94 & -4.17 & -1.55 & -1.51 \\
    \midrule
    { } & $\text{H}_\text{edge}$ & \cellcolor[rgb]{ .647,  .647,  .647}0.4700 & \cellcolor[rgb]{ .647,  .647,  .647}0.4450 & \cellcolor[rgb]{ .647,  .647,  .647}0.2220 & \cellcolor[rgb]{ .647,  .647,  .647}0.0730 & \cellcolor[rgb]{ .647,  .647,  .647}0.6180 & 0.5450 & \cellcolor[rgb]{ .647,  .647,  .647}0.5250 \\
     & $\text{H}_\text{node}$ & \cellcolor[rgb]{ .647,  .647,  .647}0.4828 & \cellcolor[rgb]{ .647,  .647,  .647}0.4283 & \cellcolor[rgb]{ .647,  .647,  .647}0.2893 & \cellcolor[rgb]{ .647,  .647,  .647}0.2206 & \cellcolor[rgb]{ .647,  .647,  .647}0.5087 & 0.5564 & \cellcolor[rgb]{ .647,  .647,  .647}0.5299 \\
    {Baseline} & $\text{H}_\text{class}$ & \cellcolor[rgb]{ .647,  .647,  .647}0.0460 & \cellcolor[rgb]{ .647,  .647,  .647}0.0000 & \cellcolor[rgb]{ .647,  .647,  .647}0.2720 & \cellcolor[rgb]{ .647,  .647,  .647}0.1000 & 0.0800 & \cellcolor[rgb]{ .647,  .647,  .647}0.0900 & 0.0300 \\
    {Homophily} & $\text{H}_\text{agg}$ & \cellcolor[rgb]{ .647,  .647,  .647}0.2712 & \cellcolor[rgb]{ .647,  .647,  .647}0.0807 & 0.7066 & 0.6170 & \cellcolor[rgb]{ .647,  .647,  .647}0.7823 & \cellcolor[rgb]{ .647,  .647,  .647}0.4172 & \cellcolor[rgb]{ .647,  .647,  .647}0.5580 \\
    { Metrics} & $\text{H}_\text{GE}$ & \cellcolor[rgb]{ .647,  .647,  .647}0.3734 & 0.9222 & 0.8388 & 0.6064 & \cellcolor[rgb]{ .647,  .647,  .647}0.6655 & \cellcolor[rgb]{ .647,  .647,  .647}0.2865 & 0.0378 \\
    & $\text{H}_\text{adj}$ & \cellcolor[rgb]{ .647,  .647,  .647}0.0366 & \cellcolor[rgb]{ .647,  .647,  .647}-0.1132 & \cellcolor[rgb]{ .647,  .647,  .647}0.0729 & \cellcolor[rgb]{ .647,  .647,  .647}0.0907 & 0.1432 & \cellcolor[rgb]{ .647,  .647,  .647}0.1010 & 0.1586 \\
    & $\text{LI}$    & \cellcolor[rgb]{ .647,  .647,  .647}0.0851 & \cellcolor[rgb]{ .647,  .647,  .647}0.0172 & \cellcolor[rgb]{ .647,  .647,  .647}0.0407 & \cellcolor[rgb]{ .647,  .647,  .647}0.0243 & 0.0025 & \cellcolor[rgb]{ .647,  .647,  .647}0.0058 & 0.0007 \\
    \midrule
    {Classifier-based } & $\text{KR}_\text{NL}$ & \cellcolor[rgb]{ .647,  .647,  .647}\textcolor[rgb]{ 1,  0,  0}{0.00} & \textcolor[rgb]{ 1,  0,  0}{0.57} & 1.00  & \cellcolor[rgb]{ .647,  .647,  .647}\textcolor[rgb]{ 1,  0,  0}{0.4083} & 0.00  & 1.00  & 0.00 \\
    {Performance Metrics} & GNB & \cellcolor[rgb]{ .647,  .647,  .647}\textcolor[rgb]{ 1,  0,  0}{0.00} & \cellcolor[rgb]{ .647,  .647,  .647}\textcolor[rgb]{ 1,  0,  0}{0.00} & 1.00  & 1.00  & 0.00  & 1.00  & 0.00 \\
    \midrule
          & ACC GCN & 82.08 $\pm$ 0.31 & 70.3 $\pm$ 0.1 & 40 $\pm$ 0.26 & 35.8 $\pm$ 0.05 & 83.26 $\pm$ 0.14 & 62.33 $\pm$ 0.23 & 60.16 $\pm$ 0.51 \\
    {GCN vs MLP2} & ACC MLP-2 & 74.68 $\pm$ 0.28 & 62.13 $\pm$ 0.1 & 36.36 $\pm$ 0.23 & 31.43 $\pm$ 0.04 & 86.62 $\pm$ 0.08 & 60.9 $\pm$ 0.11 & 64.25 $\pm$ 0.41 \\
          & \textbf{Diff Acc} & 7.40  & 8.17  & 3.64  & 4.37  & -3.36 & 1.43  & -4.09 \\
    \bottomrule
    \bottomrule
    \end{tabular}%
    }
  \label{rebuttal_tab:detaied_comparison_large_scale_datasets}%
\end{table}%


==> rebuttal_tab_small_datasets_results.tex <==
% Table generated by Excel2LaTeX from sheet 'Classifier-based'
\begin{table}[htbp]
  \centering
  \caption{Comparison on small datasets}
  \resizebox{1\hsize}{!}{
    \begin{tabular}{c|c|ccccccccc}
    \toprule
    \toprule
          &       & Cornell & Wisconsin & Texas & Film  & Chameleon & Squirrel & Cora  & CiteSeer & PubMed \\
    \midrule
          & $\text{H}_\text{edge}$ & \cellcolor[rgb]{ .647,  .647,  .647}0.5669 & 0.4480 & 0.4106 & 0.3750 & \cellcolor[rgb]{ .647,  .647,  .647}0.2795 & \cellcolor[rgb]{ .647,  .647,  .647}0.2416 & 0.8100 & 0.7362 & \cellcolor[rgb]{ .647,  .647,  .647}0.8024 \\
     & $\text{H}_\text{node}$ & 0.3855 & 0.1498 & 0.0968 & 0.2210 & \cellcolor[rgb]{ .647,  .647,  .647}0.2470 & \cellcolor[rgb]{ .647,  .647,  .647}0.2156 & 0.8252 & 0.7175 & \cellcolor[rgb]{ .647,  .647,  .647}0.7924 \\
    {Baseline} & $\text{H}_\text{class}$ & 0.0468 & 0.0941 & 0.0013 & 0.0110 & \cellcolor[rgb]{ .647,  .647,  .647}0.0620 & \cellcolor[rgb]{ .647,  .647,  .647}0.0254 & 0.7657 & 0.6270 & \cellcolor[rgb]{ .647,  .647,  .647}0.6641 \\
    {Homophily} & $\text{H}_\text{agg}$ & \cellcolor[rgb]{ .647,  .647,  .647}0.8032 & \cellcolor[rgb]{ .647,  .647,  .647}0.7768 & \cellcolor[rgb]{ .647,  .647,  .647}0.6940 & \cellcolor[rgb]{ .647,  .647,  .647}0.6822 & 0.61  & \cellcolor[rgb]{ .647,  .647,  .647}0.3566 & 0.9904 & 0.9826 & \cellcolor[rgb]{ .647,  .647,  .647}0.9432 \\
    {  Metrics} & $\text{H}_\text{GE}$ & 0.31  & 0.34  & 0.35  & 0.16  & \cellcolor[rgb]{ .647,  .647,  .647}0.0152 & \cellcolor[rgb]{ .647,  .647,  .647}0.0157 & \cellcolor[rgb]{ .647,  .647,  .647}0.1700 & \cellcolor[rgb]{ .647,  .647,  .647}0.1900 & 0.27 \\
     & $\text{H}_\text{adj}$ & 0.1889 & 0.0826 & 0.0258 & 0.1272 & \cellcolor[rgb]{ .647,  .647,  .647}0.0663 & \cellcolor[rgb]{ .647,  .647,  .647}0.0196 & 0.8178 & 0.7588 & \cellcolor[rgb]{ .647,  .647,  .647}0.7431 \\
     & $\text{LI}$    & 0.0169 & 0.1311 & 0.1923 & 0.0002 & \cellcolor[rgb]{ .647,  .647,  .647}0.048 & \cellcolor[rgb]{ .647,  .647,  .647}0.0015 & 0.5904 & \cellcolor[rgb]{ .647,  .647,  .647}0.4508 & 0.4093 \\
           \midrule
{Classifier-based } & $\text{KR}_\text{L}$ & 1.39  & 0.00  & 0.00  & \cellcolor[rgb]{ .647,  .647,  .647}\textcolor[rgb]{ 1,  0,  0}{0.7834} & 1.00  & 1.00  & 1.00  & 1.00  & \cellcolor[rgb]{ .647,  .647,  .647}0.8026 \\
    {Performance Metrics} & GNB & 0.00  & 0.00  & 0.00  & 0.00  & 1.00  & 1.00  & 1.00  & 1.00  & \cellcolor[rgb]{ .647,  .647,  .647}1.0000 \\
    \midrule
          & ACC SGC & 70.98 $\pm$ 8.39 & 70.38 $\pm$ 2.85 & 83.28 $\pm$ 5.43 & 25.26 $\pm$ 1.18 & 64.86 $\pm$ 1.81 & 47.62 $\pm$ 1.27 & 85.12 $\pm$ 1.64 & 79.66 $\pm$ 0.75 & 85.5 $\pm$ 0.76 \\
    {SGC v.s. MLP1} & ACC MLP-1 & 93.77 $\pm$ 3.34 & 93.87 $\pm$ 3.33 & 93.77 $\pm$ 3.34 & 34.53 $\pm$ 1.48 & 45.01 $\pm$ 1.58 & 29.17 $\pm$ 1.46 & 74.3 $\pm$ 1.27 & 75.51 $\pm$ 1.35 & 86.23 $\pm$ 0.54 \\
          & \textbf{Diff Acc} & -22.79 & -23.49 & -10.49 & -9.27 & 19.85 & 18.45 & 10.82 & 4.15  & -0.73 \\
    \midrule
    \multicolumn{1}{p{12.57em}|}{ } & $\text{H}_\text{edge}$ & \cellcolor[rgb]{ .647,  .647,  .647}0.5669 & 0.4480 & 0.4106 & 0.3750 & \cellcolor[rgb]{ .647,  .647,  .647}0.2795 & \cellcolor[rgb]{ .647,  .647,  .647}0.2416 & 0.8100 & 0.7362 & 0.8024 \\
     & $\text{H}_\text{node}$ & 0.3855 & 0.1498 & 0.0968 & 0.2210 & \cellcolor[rgb]{ .647,  .647,  .647}0.2470 & \cellcolor[rgb]{ .647,  .647,  .647}0.2156 & 0.8252 & 0.7175 & 0.7924 \\
    {Baseline} & $\text{H}_\text{class}$ & 0.0468 & 0.0941 & 0.0013 & 0.0110 & \cellcolor[rgb]{ .647,  .647,  .647}0.0620 & \cellcolor[rgb]{ .647,  .647,  .647}0.0254 & 0.7657 & 0.6270 & 0.6641 \\
    {Homophily} & $\text{H}_\text{agg}$ & \cellcolor[rgb]{ .647,  .647,  .647}0.8032 & \cellcolor[rgb]{ .647,  .647,  .647}0.7768 & \cellcolor[rgb]{ .647,  .647,  .647}0.6940 & \cellcolor[rgb]{ .647,  .647,  .647}0.6822 & 0.61  & \cellcolor[rgb]{ .647,  .647,  .647}0.3566 & 0.9904 & 0.9826 & 0.9432 \\
    { Metrics} & $\text{H}_\text{GE}$ & 0.31  & 0.34  & 0.35  & 0.16  & \cellcolor[rgb]{ .647,  .647,  .647}0.0152 & \cellcolor[rgb]{ .647,  .647,  .647}0.0157 & \cellcolor[rgb]{ .647,  .647,  .647}0.1700 & \cellcolor[rgb]{ .647,  .647,  .647}0.1900 & \cellcolor[rgb]{ .647,  .647,  .647}0.2700 \\
     & $\text{H}_\text{adj}$ & 0.1889 & 0.0826 & 0.0258 & 0.1272 & \cellcolor[rgb]{ .647,  .647,  .647}0.0663 & \cellcolor[rgb]{ .647,  .647,  .647}0.0196 & 0.8178 & 0.7588 & 0.7431 \\
    & $\text{LI}$    & 0.0169 & 0.1311 & 0.1923 & 0.0002 & \cellcolor[rgb]{ .647,  .647,  .647}0.048 & \cellcolor[rgb]{ .647,  .647,  .647}0.0015 & 0.5904 & \cellcolor[rgb]{ .647,  .647,  .647}0.4508 & \cellcolor[rgb]{ .647,  .647,  .647}0.4093 \\
    \midrule
    {Classifier-based } & $\text{KR}_\text{NL}$ & 0.00  & 0.00  & 0.00  & 0.00  & 1.00  & 1.00  & 1.00  & 1.00  & 1.00 \\
    {Performance Metrics} & GNB & 0.00  & 0.00  & 0.00  & 0.00  & 1.00  & 1.00  & 1.00  & 1.00  & 1.00 \\
    \midrule
          & ACC GCN & 82.46 $\pm$ 3.11 & 75.5 $\pm$ 2.92 & 83.11 $\pm$ 3.2 & 35.51 $\pm$ 0.99 & 64.18 $\pm$ 2.62 & 44.76 $\pm$ 1.39 & 87.78 $\pm$ 0.96 & 81.39 $\pm$ 1.23 & 88.9 $\pm$ 0.32 \\
    {GCN v.s. MLP2} & ACC MLP-2 & 91.30 $\pm$ 0.70 & 93.87 $\pm$ 3.33 & 92.26 $\pm$ 0.71 & 38.58 $\pm$ 0.25 & 46.72 $\pm$ 0.46 & 31.28 $\pm$ 0.27 & 76.44 $\pm$ 0.30 & 76.25 $\pm$ 0.28 & 86.43 $\pm$ 0.13 \\
          & \textbf{Diff Acc} & -8.84 & -18.37 & -9.15 & -3.07 & 17.46 & 13.48 & 11.34 & 5.14  & 2.47 \\
    \bottomrule
    \bottomrule
    \end{tabular}%
    }
  \label{rebuttal_tab:detailed_comparison_small_datasets}%
\end{table}%


==> rebuttal_tab_statistics_large_datasets.tex <==
% Table generated by Excel2LaTeX from sheet 'Classifier-based'
\begin{table}[htbp]
  \centering
  \caption{Statistics on large-scale datasets}
    \begin{tabular}{c|cc}
    \midrule
    \midrule
          & Total Error & Error Rate \\
    \midrule
    $\text{H}_\text{edge}$ & 9     & 0.64 \\
    $\text{H}_\text{node}$ & 9     & 0.64 \\
    $\text{H}_\text{class}$ & 6     & 0.43 \\
    $\text{H}_\text{agg}$ & 8     & 0.57 \\
    $\text{H}_\text{GE}$ & 6     & 0.43 \\
    $\text{H}_\text{adj}$ & 6     & 0.43 \\
    $\text{LI}$    & 6     & 0.43 \\
    \midrule
    $\text{KR}$ (NT0.5)  & 2     & 0.14 \\
    $\text{KR}$ (SST0.05) & 5     & 0.36 \\
    GNB (NT0.5) & 4     & 0.29 \\
    GNB (SST0.05) & 4     & 0.29 \\
    \bottomrule
    \bottomrule
    \end{tabular}%
  \label{rebuttal_tab:statistics_large_scale_datasets}%
\end{table}%


==> rebuttal_tab_statistics_overall.tex <==
% Table generated by Excel2LaTeX from sheet 'Classifier-based'
\begin{table}[htbp]
  \centering
  \caption{Overall statistics on small- and large-scale datasets}
   \resizebox{0.465\hsize}{!}{
      \begin{tabular}{c|cc|cc|cc}
    \toprule
    \toprule
    \multirow{3}[6]{*}{Metrics} & \multicolumn{6}{c}{Statistics on Large and Small Datasets} \\
\cmidrule{2-7}          & \multicolumn{2}{c|}{Large} & \multicolumn{2}{c|}{Small} & \multicolumn{2}{c}{Overall} \\
\cmidrule{2-7}          & \#Error &  Rate & \#Error &  Rate & \#Error &  Rate \\
    \midrule
    $\text{H}_\text{edge}$ & 9     & 0.64  & 7     & 0.39  & 16    & 0.50 \\
    $\text{H}_\text{node}$ & 9     & 0.64  & 5     & 0.28  & 14    & 0.44 \\
    $\text{H}_\text{class}$ & 6     & 0.43  & 5     & 0.28  & 11    & 0.34 \\
    $\text{H}_\text{agg}$ & 8     & 0.57  & 11    & 0.61  & 19    & 0.59 \\
    $\text{H}_\text{GE}$ & 6     & 0.43  & 9     & 0.50  & 15    & 0.47 \\
    $\text{H}_\text{adj}$ & 6     & 0.43  & 5     & 0.28  & 11    & 0.34 \\
    $\text{LI}$    & 6     & 0.43  & 7     & 0.39  & 13    & 0.41 \\
    \midrule
    $\text{KR} $ (NT0.5)  & 2     & 0.14  & 2     & 0.11  & 4     & 0.13 \\
    $\text{KR} $ (SST0.05) & 5     & 0.36  & 1     & 0.06  & 6     & 0.19 \\
    GNB (NT0.5) & 4     & 0.29  & 1     & 0.06  & 5     & 0.16 \\
    GNB (SST0.05) & 4     & 0.29  & 1     & 0.06  & 5     & 0.16 \\
    \bottomrule
    \bottomrule
    \end{tabular}%
    }
  \label{rebuttal_tab:statistics_overall}%
\end{table}%


==> rebuttal_tab_statistics_small_datasets.tex <==
% Table generated by Excel2LaTeX from sheet 'Classifier-based'
\begin{table}[htbp]
  \centering
  \caption{Statistics on small-scale datasets}
    \begin{tabular}{c|cc}
    \midrule
    \midrule
          & Total Error & Error Rate \\
    \midrule
    $\text{H}_\text{edge}$ & 7     & 0.39 \\
    $\text{H}_\text{node}$ & 5     & 0.28 \\
    $\text{H}_\text{class}$ & 5     & 0.28 \\
    $\text{H}_\text{agg}$ & 11    & 0.61 \\
    $\text{H}_\text{GE}$ & 9     & 0.50 \\
    $\text{H}_\text{adj}$ & 5     & 0.28 \\
    $\text{LI}$    & 7     & 0.39 \\
    \midrule
    $\text{KR}$ (NT0.5)  & 2     & 0.11 \\
    $\text{KR}$ (SST0.05) & 1     & 0.06 \\
    GNB (NT0.5) & 1     & 0.06 \\
    GNB (SST0.05) & 1     & 0.06 \\
    \bottomrule
    \bottomrule
    \end{tabular}%
  \label{rebuttal_tab:statistics_small_scale_datasets}%
\end{table}%

